DataOps for Societal Intelligence: a Data Pipeline for Labor Market Skills Extraction and Matching

Big Data analytics supported by AI algorithms can support skills localization and retrieval in the context of a labor market intelligence problem. We formulate and solve this problem through specific DataOps models, blending data sources from administrative and technical partners in several countries into cooperation, creating shared knowledge to support policy and decision-making. We then focus on the critical task of skills extraction from resumes and vacancies featuring state-of-the-art machine learning models. We showcase preliminary results with applied machine learning on real data from the employment agencies of the Netherlands and the Flemish region in Belgium. The final goal is to match these skills to standard ontologies of skills, jobs and occupations.

==> design_bk.tex <==

\begin{figure*}[htb]
\centering
\includegraphics[width=\textwidth]{SkillsPipelineBDE}
\caption{Big Data enables Societal and Labor Market Intelligence. The process specifies which Vs of Big Data are involved in each step (adapted from~\cite{mezzanzanica2019big})}\label{fig:comm}
\end{figure*}

The extraction of knowledge from (Big) labor market data has been addressed using the knowledge discovery in databases (KDD) approach as baseline~\cite{fayyad1996kdd} -- as shown in Figure~\ref{fig:comm}, together with the span of the Vs of Big Data throughout the process. %Needless to say, this approach can be adapted to the domain of interest, enhancing specific tasks or steps.
%Figure~\ref{fig:comm} shows KDD framed within the Societal and Labor Market Intelligence context, and the span of the Vs of Big Data throughout the process. Each key step can be adapted to the Web labor market context as follows.

\paragraph{Step 1: Select Data Sources} Each Web source is evaluated and ranked to guarantee its reliability -- e.g., vacancy publication date, update frequency, (un)structured data, privacy restrictions, etc. Heterogeneous Data sources are considered here, including but not limited to, governmental employment offices (from different regions/countries), private Websites (such as indeed.com) and social networks (such as Linkedin). At the end of the process, the data sources are selected. This step deals with the 4 Vs of Big Data including \textit{veracity}, intended as the biases, noise and/or abnormalities in data.

\paragraph{Step 2 Pre-processing Selected Data} This includes data cleansing tasks to remove noise from the data or inappropriate outliers (if any), deciding how to handle missing data, as well as removing duplicated entries. Data quality and cleaning tasks are indeed \textit{mandatory} steps of any data-driven decision-making approach for guaranteeing the trust on the overall process, intended as the "the extent to which data is accepted or regarded as true, real and credible"~\cite{mezzanzanica2019big}. This step reduces the complexity of the Big Data scenario, by addressing the \textit{variety} dimension.


\paragraph{Step 3: Transformation}
This step transforms data into a unified model, which depends on the goal of the process, by means of data reduction and projection techniques. 
%It may also include dimensionality reduction to reduce the number of variables, by keeping the most representative ones. 
It usually involves ETL (Extract, Transform, Load) techniques typical of Big Data Integration scenarios~\cite{vassiliadis2002conceptual}. %Notice that, at the end of this step, the \textit{variety} dimension related to Big Data is solved thanks to the unified model. 
Around 70\% of the effort of the overall process is spent on Data Selection, Pre-processing and Transformation, to provide input data in the amount, structure and format that suit each Data Mining task perfectly~\cite{garcia15data}. 


A crucial transformation for Societal and Labour Market Intelligence consists of extracting the important information -- i.e.,  the skills (hard and soft) in the job vacancy text. More formally, the transformation function takes a job vacancy $j_k \in J$ as input and extracts a set of skills $S_k=\{ s_1,...,s_n\}$ where $S_k \in P(S)$, the powerset of skills  $S$. Note that the skills set $S$ evolves throughout time as novel skills arise. %The skills extraction process as part of the transformation allows one to focus on the important information in the vacancies and deletes all boilerplate text which acts as noise for the further step: Data Mining.



\paragraph{Step 4: Data Mining and Machine Learning} This step requires to identify proper AI algorithms (e.g., classification, prediction, regression, clustering), searching for patterns of interest. In our context, it usually involves text classification algorithms to map vacancies/resumes into one of several predefined classes in a taxonomy or ontology of job profiles and skills, such as ISCO, ESCO and/or Competent.
%~\cite{isco12ilo}, ESCO~\cite{esco16mapping} or Competent\footnote{\url{http://production.competent.be/}}.
More formally, categorization assigns a Boolean value to each pair $(j_k,c_i)\in JxC$ -- where \textit{J} are job vacancies and \textit{C} the predefined categories (of a given taxonomy) --  \textit{true} if $j_k$ belongs to $c_i$ and \textit{false} otherwise. This categorization task can be solved through machine learning: let $J = {J_1, ..., J_n}$ be a set of job vacancies and the classification of $J$ under the taxonomy consists of $|O|$ independent problems of classifying each job vacancy $J_i\in J$ under a given taxonomy occupation code $o_i$ for $i=1...|O|$. Then, a classifier is a function $\phi : JxO \xrightarrow{} \{0,1\}$.

\paragraph{Step 5: Interpretation and Feedback} Finally, this step employs visual paradigms to represent the resulting knowledge, according to the ultimate goal. In our context, this step concerns the users' ability to understand the data. For example, public administrations might be interested in identifying the most requested occupations in a cross-border area; companies might focus on monitoring skills trend and novel, arising skills and occupations, so that they can design training paths. 


\section{Skills Extraction and Matching to enable Labour Market Intelligence}\label{analytic}

Societal analytics require the definition of a metrics model for needed measurable quantities as well as analyses over those measurable quantities; we call this an \emph{analytical model}. In the scope of this paper we define an analytical model for labour intelligence, comprised of the following measurable quantities:

\begin{enumerate}

\item \textit{$[$Required $||$ Provided$]$ Skill, type and level.} A list of skills that are necessary for a certain job-offer to be fulfilled or provided by a specific job-seeker profile.

%\item \textit{$[$Required $||$ Provided$]$ Skill-Level.} 
Also, Employers need to be able to express (or infer through analysis) their required skill types (hard / soft) and levels; similarly, job-seekers require to express their skills types and levels. In both cases, a standard Likert-scale notation can be used.

\item \textit{Skills match with ontology concepts.}

The straightforward approach here is to represent words -- skills and ontology concepts -- as vectors, by means of, e.g., word2vec ~\cite{mikolov2013efficient}. All vectors/words have certain orientation and it is possible to explicitly define their relationship with each other. 

Then the words are matched according to their distance in the vectorial space. Among different distance metrics, cosine similarity (Formula~\ref{eq:cosim}) is more intuitive and most used in word2vec. It is normalized dot product of 2 vectors and this ratio defines the angle between them. A high cosine value indicates that a skill is closely related to the job (ontology concept).


\begin{equation}
\label{eq:cosim}
\cos ({\bf t},{\bf e})= { \frac{{\bf t} {\bf e}}{ \|{\bf t}\| \|{\bf e}\|}} = \frac{ \sum_{i=1}^{n}{{\bf t}_i{\bf e}_i} }{ \sqrt{\sum_{i=1}^{n}{({\bf t}_i)^2}} \sqrt{\sum_{i=1}^{n}{({\bf e}_i)^2}} }
\end{equation}

\end{enumerate}

The last step would be the efficient enrichment of the ontology. This can be based on current vacancy data and a continuous feedback loop with domain experts. The final goal is to attain an up-to-date ontology suitable and refined for specific cross-border use. In the following we showcase the design of our AI-based solution for the crucial task of Skills Extraction to enable the aforementioned measurements and goals.  


\subsection{A ataOps Processing Solution}
\label{sub:big-data-solution}

Our solution entails a DataOps pipeline combining Big Data and Machine Learning models to process text in vacancies and resumes, and then extract the sentences containing skills. Figure~\ref{fig:training-pipeline} shows the Model Training and Prediction pipelines, detailed below.

\paragraph{Data Pre-processing}

This constitutes a key preparatory step given the premise \textit{garbage in, garbage out}. Input data must be provided in the amount, structure and format that suit each Data Mining task perfectly. Unfortunately, real-world databases are highly influenced by negative factors such the presence of noise, multi-valued attributes, inconsistent and superfluous data and huge sizes in both dimensions, examples and features. Thus, low-quality data will lead to low-quality  performance and results~\cite{mierswa2006yale}. Data Pre-processing may feature several tasks, typically including Data Cleaning, Transformation, Integration, Normalization, Missing Data Imputation and Noise Identification~\cite{garcia15data}.



In our particular case, given the characteristics of the input (vacancies text), the following text  pre-processing steps are necessary:

\begin{itemize}
    \item Distinguish end-of-sentence periods ( . ) from others (e.g. abbreviations, acronyms, websites, etc.).
    \item Distinguish end-of-sentence line breaks (\textit{\textbackslash	n}) from spurious ones by looking ahead to see if the \textbackslash	n is followed by a capital letter.
    \item Delete unnecessary spacing/tabbing.
    \item Identify some special cases that use two spaces or tabs to mark the start of a new line/sentence.
    \item Identify and replace certain characters used as bullet points (such as hyphens or dashes).
    \item Some Vacancies use the letter 'o' as bullet points. No solution for removing this without affecting the splitting of the majority of other sentences.
    \item Trim leading and trailing whitespaces.
    \item Replace quotation marks ( " ) with apostrophes ( ' ) for Dutch plurals/abbreviations (e.g. collega's, zo'n). 
    \item Filter stopwords, generally the most common words with little lexical meaning, such as pronouns, articles and functors.
\end{itemize}

The output of this step is a list of processable sentences, ready to be used by the Machine Learning algorithm. 

\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{TrainingPrediction.pdf}
  \caption{Model training and prediction pipelines for skills extraction and matching.}\label{fig:training-pipeline}
\end{figure*}

\paragraph{Sentences Annotation for Learning}


Each sentence in the training set must be annotated by domain experts: the ones that contain a skill are annotated with a 1, otherwise with a 0.

In the case of some ambiguous sentences, we created a codebook with help of the domain experts as an aid to identify and correctly annotate the sentences representing a skill, with the following, previously agreed definitions:

 \textbf{Hard skill}: Is a professional skill, activity or knowledge. These are related to functions, processes and roles in organizations and are needed in practice to successfully complete a specific task. In other words; good hard skills ensure an invitation to a job interview. For example:

\textit{Your work consists of checking and controlling cleaning activities of the chambermaids, opening and / or closing your service, communication with the reception and / or guests and light administrative work.
}

An example of vacancy sentences without hardskill:

 \textit{   It is an international company that provides management, advisory and engineering services on socially relevant issues related to mobility, environment \& space, buildings and water.}

 \textbf{Soft skill}: Is a personal, emotional, social or intellectual skill, also called \textit{behavioral skill} or competence. Soft skills are often seen as good-to-have in addition to the hard skills. These are about how someone comes across to the employer and in this way ensure that the choice falls on that person or not after a job interview. For example: 

 \textit{   You are able to maintain customer relationships, identify opportunities and utilize and expand your network;}




\paragraph{Model Training}

This happens on two steps, namely: pre-training from unlabeled text and then supervised training from labeled text. 


First the model is trained on unlabeled data over different pre-training tasks. This reduces the need for many heavily-engineered task-specific architectures. Pre-trained models can be fine-tuned with just one additional output layer to create state-of-the-art models for a wide range of tasks, such as question answering and language inference, without substantial task-specific architecture modifications~\cite{devlin2018bert}.


\paragraph{Supervised Training (fine-tunning)}

A training set is given and the objective is to form a description that can be used to predict unseen examples. This training set is typically a set of labeled instances~\cite{garcia15data}. 

For this is also necessary to properly tokenize the text we are planning to work with, according to the pre-processing steps and a built-in tokenizer. Afterwards all the input data ('train' data) is converted into the format that the model understands -- typically in the form of csv or tsv files, containing the columns with the annotations, the vacancies/resumes and skills ids for traceability, and the actual sentence text.

At this point the model can be actually trained for the needed purposes. Early stopping with a configurable number of epochs is recommended, as the training theoretically should finish when the model achieves the optimal state under the setup conditions, avoiding overfitting.

Afterwards, the accuracy can be verified using the 'dev' validation dataset, a labeled set not directly used for training. Note that currently a small set of manually annotated data is used to train the model. It has been noticed that increasing the training set even by ~500-600 examples (taking them from the validation set) had in few cases boosted the predictions accuracy by 3-5\%.

All in all, the output of this process is the trained model which can be used for further predictions. Note that, compared to pre-training, fine-tuning is relatively inexpensive. All of the results in the following section can be replicated in at most 1 hour on a single Cloud TPU, or a few hours on a GPU, starting from the exact same pre-trained model.

\paragraph{Predictions with the Pre-trained ML Model}

At this point the model is ready to make predictions, according to the pipeline depicted in Figure~\ref{fig:training-pipeline}.  Recall that the goal of the pipeline is to classify (predict) sentences describing skills from a vacancy text. The nature of classification is to discriminate examples from others, attaining as a main application a reliable prediction: once we have a model that fits the past data (training), if the future is similar to the past, then we can make correct predictions for new instances~\cite{garcia15data}. 

The first step of input text pre-processing is equivalent to the one performed for model training. Then the sentences extracted from the processed vacancies/resumes text are given as input to the model, pre-trained and fine-tuned during the training pipeline. 

Then the unlabeled sentences extracted from vacancies text are given as input in the proper tsv/csv format. The output contains the predictions for each sample,  with the original text, ids and class probabilities (whether the sentence contains a skill or not).
